Security of XCB and HCTR

Tweakable Enciphering Scheme (TES) is a length preserving scheme which provides confidentiality and admissible integrity. XCB (Extended Code Book) is a TES which was introduced in 2004. In 2007, it was modified and security bound was provided. Later, these two versions were referred to as XCBv1 and XCBv2 respectively. XCBv2 was proposed as the IEEE-std 1619.2 2010 for encryption of sector oriented storage media. In 2013, first time Security bound of XCBv1 was given and XCBv2's security bound was enhanced. A constant of $2^{22}$ appears in the security bounds of the XCBv1 and XCBv2. We showed that this constant of $2^{22}$ can be reduced to $2^{5}$. Further, we modified the XCB (MXCB) scheme such that it gives better security bound compared to the present XCB scheme. We also analyzed some weak keys attack on XCB and a type of TES known as HCTR (proposed in 2005). We performed distinguishing attack and the hash key recovery attack on HCTR. Next, we analyzed the dependency of the two different keys in HCTR.

==> preambles/front_title.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Contents: The title page
% $Id: title.tex,v 1.2 2003/03/19 20:57:47 oetiker Exp $
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \ifx\pdfoutput\undefined % We're not running pdftex
% \else
% \pdfbookmark{Title Page}{title}
% \fi
\newtcbox{\mybox}{enhanced,frame hidden,colback= ,boxrule=0.5pt,arc=4pt,
boxsep=0pt,left=6pt,right=6pt,top=6pt,bottom=6pt}
\newlength{\centeroffset}
\setlength{\centeroffset}{-0.5\oddsidemargin}
\addtolength{\centeroffset}{0.5\evensidemargin}

%\addtolength{\textwidth}{-\centeroffset}
%\pagecolor{Emerald}\afterpage{\nopagecolor}
\thispagestyle{empty}
\vspace*{\stretch{1}}
\noindent\hspace*{\centeroffset}\makebox[0pt][l]{
{\LARGE \textbf{ \textsc{
\begin{tcolorbox}[enhanced,frame hidden, colback=Peach,boxrule=0.5pt,arc=4pt,
boxsep=0pt,left=10pt,right=10pt,top=6pt,bottom=6pt]
\begin{center}
\color{white} Collision-free Routing Problem with Restricted L-path
\end{center}
\end{tcolorbox}
}}}}
%\vspace*{\stretch{1}}
%\noindent\hspace*{\centeroffset}\makebox[0pt][l]{
%\begin{minipage}{\textwidth}
%\flushright
%{\centering \huge \sf 
%\begin{spacing}{.8}
%\mybox{Collision-free Routing Problem with Restricted L-path}
%\end{spacing}
%}
%\noindent\rule[-1ex]{\textwidth}{5pt}\\[2.5ex]
%% \hfill\emph{\Large Or \LaTeXe{} in \pageref{verylast} minutes}
%\end{minipage}}

\vspace*{13cm}
% \noindent\rule[-1ex]{\textwidth}{1pt}\\[2.5ex]
\noindent\hspace*{\centeroffset}\makebox[0pt][l]{\begin{minipage}{\textwidth}
\flushright
{\sf
{\Large \bf Jammigumpula Ajay Kumar}\\[3ex]} 
%{\sf \emph{February 2006}}
\end{minipage}}

%\addtolength{\textwidth}{\centeroffset}
\vspace{\stretch{2}}


%\pagebreak

\endinput
%\begin{titlepage}
%    \begin{center}
%        \vspace*{1cm}
%        
%        \Huge
%        \textbf{Collision-free Routing Problem with Restricted L-path}
%        
%        \vspace{0.5cm}
%        %\LARGE
%        %Thesis Subtitle
%        
%        \vspace{1.5cm}
%        
%        \textbf{Jammigumpula Ajay Kumar}
%        
%        \vfill
%        
%        Dissertation Submitted In Partial Fulfilment Of The Requirements For The Degree Of\\
%        Master of Technology
%        
%        \vspace{0.8cm}
%        
%        \begin{figure}[htbp]
%{\centering \resizebox*{!}{3.5cm}{\includegraphics{isilogo.png}} \par}
%\end{figure}
%\vspace {0.3in}
%        
%        \Large
%        Department Name\\
%        University Name\\
%        Country\\
%        Date
%        
%    \end{center}
%\end{titlepage}
